Evaluating the Evaluation Metrics for Style Transfer: A Case Study in Multilingual Formality Transfer

While the field of style transfer (ST) has been growing rapidly, it has been hampered by a lack of standardized practices for automatic evaluation. In this paper, we evaluate leading ST automatic metrics on the oft-researched task of formality style transfer. Unlike previous evaluations, which focus solely on English, we expand our focus to Brazilian-Portuguese, French, and Italian, making this work the first multilingual evaluation of metrics in ST. We outline best practices for automatic evaluation in (formality) style transfer and identify several models that correlate well with human judgments and are robust across languages. We hope that this work will help accelerate development in ST, where human evaluation is often challenging to collect.

==> tables/cross-metric.tex <==
\begin{figure*}[!t]
    \centering

    \subfigure[\textsc{en}]{\includegraphics[width=0.24\textwidth]{figs/en_meaning_corellations.png}} 
    \subfigure[\textsc{fr}]{\includegraphics[width=0.24\textwidth]{figs/it_meaning_corellations.png}} 
    \subfigure[\textsc{it}]{\includegraphics[width=0.24\textwidth]{figs/fr_meaning_corellations.png}} 
    \subfigure[\textsc{pt}]{\includegraphics[width=0.24\textwidth]{figs/pt_meaning_corellations.png}} 
    \caption{Cross-metric correlations for meaning preservation automatic evaluation metrics. Mode-based metrics marked with $*$ use \textsc{xlm-r} while markers $\sim$ use m\textsc{bert} as the base pre-trained language model.}
    \label{fig:cross_metric_meaning}
\end{figure*}

\begin{figure*}[!t]
    \centering

    \subfigure[\textsc{en}]{\includegraphics[width=0.24\textwidth]{figs/en_cross-metric_corellations.png}} 
    \subfigure[\textsc{fr}]{\includegraphics[width=0.24\textwidth]{figs/it_cross-metric_corellations.png}} 
    \subfigure[\textsc{it}]{\includegraphics[width=0.24\textwidth]{figs/fr_cross-metric_corellations.png}} 
    \subfigure[\textsc{pt}]{\includegraphics[width=0.24\textwidth]{figs/pt_cross-metric_corellations.png}} 
    \caption{Cross-metric correlations for fluency and formality automatic evaluation metrics.
    Mode-based metrics marked with $*$ use \textsc{xlm-r} while markers $\sim$ use m\textsc{bert} as the base pre-trained language model. \textsc{f.reg} refers to formality regression models, \textsc{ppl} to perplexity, and \textsc{ll} to likelihood.
    }
    \label{fig:cross_metric_fluency_formality}
\end{figure*}

==> tables/formality.tex <==
\begin{table*}[!t]
    \centering
    \begin{tabular}{ll@{\hskip 0.2in}cccc@{\hskip 0.2in}cccc}
    
    & & \multicolumn{4}{c}{\textbf{\textsc{regression}} (Spearman)} & \multicolumn{4}{c}{\textbf{\textsc{classification}} (F$1$)}\\
    
    \rowcolor{gray!10}
    \multicolumn{2}{c}{\textbf{\textsc{method}}} & \textbf{\textsc{en}} & \textbf{\textsc{it}} & 
    \textbf{\textsc{pt}} & \textbf{\textsc{fr}} & \textbf{\textsc{en}} & \textbf{\textsc{it}} & \textbf{\textsc{pt}} & \textbf{\textsc{fr}} \\
    

    \multirow{3}{*}{m\textsc{bert} \Bigg\{} 
    
    & \textsc{translate-train} & $0.656$ & $0.490$ & $0.611$ & $0.478$ & $\mathbf{0.903}$ &  $0.831$ &	$0.851$ & $0.819$\\
    & \textsc{translate-test}  &  $-$    & $0.450$ & $0.603$ & $0.390$ &  $-$  & 	$0.793$ &  $0.819$ &	$0.734$ \\
    & \textsc{zero-shot}       &  $-$   & $0.514$ & $0.643$ & $0.512$ &  $-$  &  $0.878$ & $0.867$ &	$0.838$\\
    
    \addlinespace[0.3cm]
    
    \multirow{3}{*}{\textsc{xlm-r} \Bigg\{} 
    
    & \textsc{translate-train} &  $\mathbf{0.670}$ & $0.553$ &$0.626$ &$0.521$ & $0.899$ &	$0.836$ & $0.871$ &	$0.837$\\
    & \textsc{translate-test}  &  $-$     & $0.510$ & $0.610$ & $0.368$ &  $-$    & $0.800$ & $0.823$ &	$0.737$\\
    & \textsc{zero-shot}       & $-$     & $\mathbf{0.608}$ & $\mathbf{0.716}$ & $\mathbf{0.586}$ &  $-$    & $\mathbf{0.891}$ & $\mathbf{0.903}$ &	$\mathbf{0.862}$\\
    
    \end{tabular}
    \caption{Formality transfer evaluation}
    \label{tab:style_metrics_correlations_with_human}
\end{table*}
%
\begin{figure*}[!t]
    \centering
    \subfigure[\textsc{en}]{\includegraphics[width=0.24\textwidth]{figs/en.png}} 
    \subfigure[\textsc{pt}]{\includegraphics[width=0.24\textwidth]{figs/pt.png}} 
    \subfigure[\textsc{fr}]{\includegraphics[width=0.24\textwidth]{figs/fr.png}} 
    \subfigure[\textsc{it}]{\includegraphics[width=0.24\textwidth]{figs/it.png}} 
    \caption{Number of formal vs. informal predictions of binary classifiers for each formality bins. Binary classifiers are biased towards outputing formal predictions for non-\english languages, while their performance degrades when moving closer to more neutral formality levels.}
    \label{fig:counts_regression}
\end{figure*}

==> tables/meaning_preservation_metrics.tex <==
\begin{table*}[!ht]
    \centering
    \scalebox{0.6}{
    \begin{tabular}{cl@{\hskip 0.5in}lll@{\hskip 0.5in}lll@{\hskip 0.5in}lll@{\hskip 0.5in}lll}

    
    
    & & \multicolumn{3}{c}{self-\textsc{bleu} ($\shneg$)} & \multicolumn{3}{c}{\textsc{mbert score} ($\shneg$)} & \multicolumn{3}{c}{\textsc{perplexity} ($\shpos$)} & \multicolumn{3}{c}{multi-\textsc{bleu} ($\shneg$)}\\ 
    
    & \textbf{Method}         & \portuguese & \italian   & \french   & \portuguese & \italian & \french   & \portuguese & \italian & \french  & \portuguese & \italian & \french\\\
    & \textsc{gold standard}  & \ptsix$23.8$ & \itseven$16.2$  & \freight$19.2$     & \ptzero$-0.48$ & \itzero$-0.39$ & \frzero$-0.42$ & \ptzero$5.32$ & \itone$5.84$ & \frzero$4.70$ & \fil      & \fil        & \fil \\
    & \textsc{copy}           & \fil         & \fil        & \fil      & \ptsix$-1.67$   & \iteight$-1.94$  & \frsix$-2.04$  & \pteight$8.77$   & \iteight$8.58$  & \frsix$8.36$  & \ptfive$46.2$  & \itfive$40.2$ & \frfive$44.3$\\
    & \textbf{\textsc{rule-based}}         & \ptone$\mathbf{79.8}$ & \itone$\mathbf{83.4}$ & \frone$\mathbf{85.4}$ &  \ptfive$-1.33$  & \itfive$-1.41$ & \frfive$-1.59$ & \ptseven$7.21$  & \itsix$7.24$ & \frfive$7.07$ &  \ptthree$53.1$ & \itone$\mathbf{43.1}$  & \frthree$46.1$   \\
    & \textbf{\textsc{round-trip mt}}           & \ptfive$33.0\SG$ & \itfive$39.7\SG$ & \frfive$32.5\SG$ & \ptthree$-1.10\SG$ & \itfour$-1.27\SG$ & \frfour$-1.20\SG$ & \ptthree$6.27\SG$ & \itfour$6.84\SG$ & \frfour$6.03\SG$ & \ptsix$43.0\SG$   & \itsix$34.5\SG$  & \frsix$41.4\SG$ \\  
    & \textbf{\textsc{translate train tag}}          & \ptthree$60.9\SG$& \itthree$57.0\SG$ & \frthree$51.8\SG$  & \pttwo$-0.96\SG$  & \itone$\mathbf{-0.90}\SG$   & \frtwo$-0.94\SG$   & \pttwo$5.89\SG$  & \ittwo$6.03\SG$   & \frtwo$5.36\SG$ & \ptfour$52.4\sg$  & \itthree$42.6$  & \frfour$44.9\sg$ \\
    \rot{\rlap{~Automatic}}
    & \textbf{\textsc{multi-task tag-style}}   & \ptfour$57.6\SG$ & \itfour$54.6\SG$  & \frfour$48.8\SG$ & \ptone$\mathbf{-0.91}\SG$  & \ittwo$-0.91\SG$   & \frone$\mathbf{-0.86}\SG$   & \ptone$\mathbf{5.85}\SG$  & \itzero$\mathbf{5.83}\SG$  & \frone$\mathbf{5.19}\SG$ & \ptone$\mathbf{55.0}\sg$   & \itfour$42.5$   & \frtwo$47.9\sg$ \\
    & \textbf{\textsc{backtranslate}}     & \pttwo$75.7\SG$  & \ittwo$68.8\SG$   & \frtwo$71.9\SG$   & \ptfour$-1.12\SG$ & \itthree$-1.07\SG$ & \frthree$-1.19\SG$ & \ptfour$6.39\SG$ & \itthree$6.28\SG$ & \frthree$5.93\SG$ & \pttwo$54.6\SG$   & \ittwo$42.9$    & \frone$\mathbf{48.3}\SG$\\
    
    %\addlinespace[0.3cm]
    & \textbf{\textsc{unmt}} & \pteight$15.3\SG$ & \iteight$15.1\SG$ & \frseven$19.7\SG$ & \ptseven$-1.74\SG$ & \iteight$-1.84\SG$ & \freight$-1.91\SG$ & \ptsix$6.42\SG$ & \itsix$6.40\SG$ & \frfive$6.61\SG$ & \pteight$14.8\SG$ & \iteight$11.5\SG$ & $17.0\SG$ \\
    & \textbf{\textsc{dlsm}} & \ptseven$20.4\SG$ & \itsix$19.6\SG$ & \frsix$21.3\SG$ & \ptseven$-1.84\SG$ & \itsix$-1.61\SG$ & \freight$-1.90\SG$ & \ptseven$6.97\SG$ & \itseven$7.45\SG$ & \frfive$6.97\SG$ & \ptseven$18.4\SG$ & \itseven$12.4\SG$ & \freight$17.4\SG$ \\

    %\addlinespace[0.2cm]
    & \textbf{\textsc{unmt (in-domain)}} & \fil  & \fil  & \frthree$52.8\SG$ & \fil  & \fil  & \frseven$-1.71\SG$ & \fil & \fil & \frfive$5.69\SG$ & \fil  & \fil & \frseven$35.0\SG$ \\
    & \textbf{\textsc{dlsm (in-domain)}} & \fil  & \fil  & \frtwo$71.2\SG$ & \fil & \fil & \frsix$-1.66$ & \fil & \fil  & \frsix$6.78\SG$ & \fil  & \fil  & \frsix$42.1\SG$ \\  

    \addlinespace[3.5em]
 
    
    &    & \multicolumn{3}{l}{\textsc{mean. preserv.} ($\shneg$)} & \multicolumn{3}{c}{\textsc{formality} ($\shneg$)} & \multicolumn{3}{c}{\textsc{fluency} ($\shneg$)} & \multicolumn{3}{c}{\textsc{overall} ($\shneg$)} \\ 
    &         & \portuguese      & \italian        & \french        & \portuguese     & \italian         & \french         & \portuguese & \italian & \french & \portuguese & \italian & \french\\\
    & \textsc{gold standard}  & \ptfive$4.88$    & \itfive$5.18$   & \frthree$5.08$ & \ptzero$+0.66$   & \itzero$+1.46$    & \frzero$+1.14$   & \ptzero$4.54$ & \itzero$4.79$  & \frzero$4.51$ & \fil & \fil & \fil\\
    & \textsc{copy}           & \fil             & \fil            & \fil           & \ptsix$-1.18$   &  \itsix$-1.06$   & \frsix$-0.75$   & \ptsix$3.91$  & \itfive$4.09$  & \frfive$3.88$  & \fil & \fil & \fil \\
    & \textbf{\textsc{rule-based}}     & \ptone$\mathbf{5.70}$     & \itthree$\mathbf{5.96}$  & \frone$\mathbf{5.95}$   & \ptfive$-0.51$  &  \itfive$-0.36$  & \frfive$-0.36$  & \ptfive$4.06$ & \itthree$4.24$ & \frfour$3.94$     & \ptfour$2.81$ & \itone$3.23$ & \frthree$2.89$\\
    & \textbf{\textsc{round-trip mt}}       & \ptsix$4.80\SG$     & \itsix$5.03\SG$   & \frsix$4.50\SG$    & \ptone$\mathbf{-0.17}\SG$   &  \itfour$-0.34$  & \frone$\mathbf{+0.25}\SG$      & \ptfour$4.07$ & \itsix$4.03\sg$   & \frthree$3.97$ & \ptthree$2.89$ & \itfour$2.54\SG$ & \frtwo$2.94$\\
          \rot{\rlap{~Human}}
    & \textbf{\textsc{translate train tag}}        & \ptfour$4.97\SG$   & \itfive$5.18\SG$   & \frfive$4.56\SG$  & \pttwo$-0.26\sg$   & \itone$\mathbf{+0.07}\sg$      & \frtwo$+0.10\SG$  & \ptthree$4.15$ & \ittwo$4.33$  & \frsix$3.84$   & \ptone$3.03\sg$ & \ittwo$3.02\sg$ & \frfour$2.83$\\
    & \textbf{\textsc{multi task tag-style}} &  \ptthree$5.07\SG$ & \itfive$5.18\SG$   & \frfour$4.81\SG$  & \ptthree$-0.27$ &  \ittwo$+0.01\sg$     & \frthree$+0.05\SG$   & \ptthree$4.15$ & \itfour$4.22$ & \frfive$3.88$  & \ptzero$\mathbf{3.24}\SG$ & \itthree$2.93\sg$ & \frzero$\mathbf{3.19}\sg$ \\
    & \textbf{\textsc{backtranslate}}   &  \pttwo$5.54\SG$   & \itfour$5.72\SG$   & \frtwo$5.59\SG$   & \ptfour$-0.49$  &  \itthree$-0.16$  & \frfour$-0.13$         & \pttwo$\mathbf{4.19}\sg$   & \itone$\mathbf{4.37}$  & \frtwo$\mathbf{4.00}$   & \pttwo$3.01\sg$ & \itzero$\mathbf{3.25}$ & \frone$3.13\SG$\\
    
    \end{tabular}}
    \caption{Automatic and human evaluation results for multilingual \fst. 
    $\sg$ denotes statistical significance differences compared to \textsc{rule-based} ($p<0.05$).
    \textsc{nmt}-based results are ensembles of $4$ systems; unsupervised models are average results across $4$ reruns. Darker colors denote higher rankings, bold numbers denote best systems.}
    \label{tab:results_all}\vspace{-0.5cm}
\end{table*}
%




==> tables/overall.tex <==
\begin{figure*}[!t]
    \centering

    \subfigure[\textsc{en}]{\includegraphics[width=0.24\textwidth]{tables/system_rankings/en_per_dimension.pdf}} 
    \subfigure[\textsc{fr}]{\includegraphics[width=0.24\textwidth]{tables/system_rankings/fr_per_dimension.pdf}} 
    \subfigure[\textsc{it}]{\includegraphics[width=0.24\textwidth]{tables/system_rankings/it_per_dimension.pdf}} 
    \subfigure[\textsc{pt}]{\includegraphics[width=0.24\textwidth]{tables/system_rankings/pt_per_dimension.pdf}} 
    \caption{Difference in relative ranking of different systems between humans judgments and automatic metrics for different evaluation dimensions. Each marker represents a system. A perfect metric should should place all systems in the dashed line (i.e., induce same ranking as the human evaluation). \sts, s-\bleu and ch\textsc{rf} are compared with rankings of systems with respect to meaning preservation, r-\bleu (reference-\bleu) compares with overall evaluation rankings, formality rankings based on formality regression scores from \textsc{xlm-r} (*\textsc{f.reg} (Zero-shot)) compared with ranking for formality style, and pseudo-perplexity from \textsc{xlm-r} (*\textsc{ppl}) compares with fluency human rankings.\eb{Will think of a better way to represent this.}}
    \label{fig:system_ranking_per_dimenstion}
\end{figure*}

==> tables/status.tex <==
\renewcommand{\arraystretch}{1.05}
\begin{table*}[!t]
    \centering
    \scalebox{0.65}{
    \begin{tabular}{llllr@{\hskip 0.4in}llll@{\hskip 0.4in}lllr@{\hskip 0.4in}lr}
    
    
    \textbf{\textsc{paper \texttt{id}}} & \multicolumn{4}{c}{\textbf{\textsc{style}}} & \multicolumn{4}{c}{\textbf{\textsc{meaning}}} & \multicolumn{4}{c}{\textbf{\textsc{fluency}}} & \multicolumn{2}{c}{\textbf{\textsc{overall}}}  \\
    \addlinespace[0.2em]
    \toprule
    \addlinespace[0.5em]
    
    & \texttt{type} & \texttt{metric} &  \texttt{model} &   & \texttt{type}  & \texttt{metric} &  \texttt{model} &  & \texttt{type} & \texttt{metric} &  \texttt{model} &  & \texttt{metric} &  \\
    \addlinespace[0.3em]

     %2018 
     \textbf{\texttt{[1]}}      & \textsc{reg} & \textsc{avg}    & Linear reg. &  \xmark & \textsc{cls} & \textsc{{avg}} & \cnn &  \cmark & \textsc{reg} & \textsc{avg} & Linear reg. & \xmark & r-\bleu & \cmark\\
    %2019
    \textbf{\texttt{[2]}}   & \C   &  \C   & \C & \C & \C  & \C & \C  & \C & \C & \C & \C & \C & r-\bleu & $-$  \\  % 
    % 2019
    \textbf{\texttt{[3]}}   & \textsc{cls} & \acc &  \cnn &  $-$   & \C & r-\bleu     & \C & $-$ & \C & \C & \C & \C    & \textsc{gm(s,m)} & $-$ \\  
    % 2019
    \textbf{\texttt{[4]}}   & \textsc{cls} & \acc  & \cnn & \xmark  & \C & r-\bleu    & \C &  \cmark & \C & \C & \C  & \C &  \textsc{gm(s,m)} &  \cmark  \\
    % 2019
    \textbf{\texttt{[5]}}   & \textsc{cls} & \acc  & \cnn &  \xmark & \C & r-\bleu & \C &  \cmark & \C & \C & \C & \C & \C & \C  \\
    % 2019
    \textbf{\texttt{[6]}}   & \textsc{cls} & \acc   & \lstm & $-$ & \textsc{cls} & \textsc{{avg}} & \bert &  $-$ & \C & \C & \C & \C  &  r-\bleu &   $-$ \\
    % 2019
    \textbf{\texttt{[7]}}   & \C    & \C    & \C & \C & \C & \C & \C & \C & \C & \C & \C & \C & r-\bleu & $-$ \\
    % 2019
    \textbf{\texttt{[8]}}   & \textsc{cls} & \acc  & \cnn &  $-$ & \C & \C & \C & \C & \C & \C & \C & \C & \C & \C  \\
    % 2019
   \textbf{\texttt{[9]}}    & \textsc{cls} & \acc  & \lstm & $-$ & \textsc{emb} & \textsc{sim} & \C &  $-$ & \textsc{lm} & \ppl & \textsc{rnn} &  $-$ & \textsc{f$1$(s,m)} & $-$ \\
    % 2020
   \textbf{\texttt{[10]}}   & \textsc{cls} & \acc  & \rob  & \xmark & \textsc{emb} & \textsc{sim} & \C & \cmark & \textsc{lm} & \ppl & \rob   &  $-$  & \textsc{j(s,m,f)} & \cmark\\  
    % 2020
   \textbf{\texttt{[11]}}   & \textsc{cls} & \acc  & \cnn &  \xmark & \C & r-\bleu & \C &  \xmark & \C & \C & \C & \C & \textsc{f$1$(s,m)} & $-$ \\
    % 2020
    \textbf{\texttt{[12]}}  & \textsc{cls} & \acc   &  \gru &  \xmark & \C & \C & \C & \C &  \textsc{cls} &  \textsc{avg} & Linear reg. & \xmark & r-\bleu & \xmark\\
    % 2020
    \textbf{\texttt{[13]}}  & \textsc{cls} & \acc   & \bert & \cmark & \C & r-\bleu & \C &  \cmark & \textsc{lm} & \ppl &  \kenlm & \xmark & \textsc{gm(s,m,f)} &  $-$\\
    % 2020
    \textbf{\texttt{[14]}}  & \C   & \C    & \C     & \C  & \C & \C  & \C & \C & \C &  \C & \C & \C  & r-\bleu & $-$  \\
    % 2020 
    \textbf{\texttt{[15]}}  & \textsc{cls} & \acc  & \textsc{fastText} & \cmark & \C & r-\bleu & \C &  \cmark & \textsc{lm} & \ppl & \gpt & \cmark & \C & \C \\
    % 2020
    \textbf{\texttt{[16]}}  & \textsc{cls} & \acc  & \cnn     & $-$  & \C & r-\bleu & \C & $-$ & \textsc{lm} & \ppl & \lstm & $-$ & \C & \C \\
    % 2020
    \textbf{\texttt{[17]}}  & \textsc{cls} & \acc  & \cnn & \cmark   & \C & r-\bleu & \C &  \cmark & \C & \C & \C & \C & \C & \C \\
    % 2020
    \textbf{\texttt{[18]}}  & \textsc{cls} & \acc  & \cnn & \cmark & \C & r-\bleu & \C &  \cmark & \C & \C & \C & \C & \textsc{gm|hm(s,m)} &   \cmark  \\  %
    % 2020
   \textbf{\texttt{[19]}}   & \textsc{cls} & \acc  & \gru   & $-$ & \textsc{cls} & \textsc{{avg}} &  \bert &  $-$ & \C & \C & \C & \C & r-\bleu &  \cmark \\
    % 2020
    \textbf{\texttt{[20]}}  & \textsc{cls} & \acc  & \rob &  $-$ & \C & r-\bleu & \C &  $-$ & \textsc{lm} & \ppl &  \gpt & $-$ & \textsc{gm|hm(s,m)} & $-$ \\
    % 2020
    \textbf{\texttt{[21]}}  & \textsc{cls} & \acc  & \cnn  & $-$     & \C & r-\bleu & \C &  \cmark & \textsc{lm} & \ppl & \gpt & \cmark & \C & \C\\
    % 2021
    \textbf{\texttt{[22]}}  & \C   & \C  & \C  & \C     & \C & \C & \C & \C & \C & \C  & \C & \C & r-\bleu &  $-$  \\
    % 2021
    \textbf{\texttt{[23]}}  & \textsc{reg} & \textsc{avg}  & \bert    & \xmark & \C & s-\bleu & \C &  \cmark & \textsc{lm} & \ppl & \kenlm & \xmark & r-\bleu &  \xmark  \\

    \end{tabular}}
    \caption{Details on automatic evaluation practices of prior work for \fost. For each dimension, \cmark \ \ and \xmark \ \ denote whether the best ranking system based on the automatic evaluation agrees or disagrees with the one pointed by the human evaluation; $-$ denotes that no human evaluation is conducted. \reg stands for regression, \textsc{cls} for classification, \textsc{acc} for accuracy, \textsc{avg} for average score, \textsc{emb} for embedding-based, \textsc{lm} for language model, \textsc{gm} or \textsc{hm} for geometric or harmonic mean, and \textsc{j} for corpus-level product. The mappings between each paper \textsc{\texttt{id}} and its corresponding citation is included in Table~\ref{tab:status_mapping}.}
    \label{tab:status}
\end{table*}
%
\begin{table}[!t]
    \centering
    \scalebox{0.65}{
    \begin{tabular}{l@{\hskip 0.5in}l@{\hskip 0.8in}l}
    
    
    \textbf{\textsc{paper \texttt{id}}} & \textbf{\textsc{citation}} & \textbf{\textsc{language}} \\
    \addlinespace[0.2em]
    \toprule
    \addlinespace[0.5em]
    
     %2018 
    \textbf{\texttt{[1]}} &  \citet{rao-tetreault-2018-dear}         &   \english \\
    %2019
    \textbf{\texttt{[2]}} & \citet{kajiwara-2019-negative}          &   \english \\  % 
    % 2019
    \textbf{\texttt{[3]}} & \citet{li-etal-2019-domain}             & \english \\  
    % 2019
    \textbf{\texttt{[4]}} & \citet{ijcai2019-711}                   & \english \\
    % 2019
    \textbf{\texttt{[5]}} & \citet{shang-etal-2019-semi}            &  \english \\
    % 2019
    \textbf{\texttt{[6]}} & \citet{wang-etal-2019-harnessing}       &  \english \\
    % 2019
    \textbf{\texttt{[7]}} &  \citet{hybrid}                          &  \english \\
    % 2019
    \textbf{\texttt{[8]}} & \citet{korotkova}                       & \english, \textsc{et}, \textsc{lv}  \\
    % 2019
    \textbf{\texttt{[9]}} &  \citet{gong}                            & \english \\
    % 2020
    \textbf{\texttt{[10]}} & \citet{krishna-etal-2020-reformulating} & \english \\  
    % 2020
    \textbf{\texttt{[11]}} & \citet{abhilasha}                       &  \english \\
    % 2020
    \textbf{\texttt{[12]}} & \citet{Wu_Wang_Liu_2020}                &  \english \\
    % 2020
    \textbf{\texttt{[13]}} & \citet{ijcai2020-526}                   & \english \\
    % 2020
   \textbf{\texttt{[14]}} &  \citet{zhang-etal-2020-parallel}        &  \english \\
    % 2020
    \textbf{\texttt{[15]}} & \citet{goyal}                           & \english \\
    % 2020
    \textbf{\texttt{[16]}} & \citet{he2020a}                         &  \english \\
    % 2020
   \textbf{\texttt{[17]}} &  \citet{chen}                            & \english \\
    % 2020
    \textbf{\texttt{[18]}} & \citet{zhou}                            & \english \\  %
    % 2020
    \textbf{\texttt{[19]}} & \citet{wang-etal-2020-formality}        & \english \\
    % 2020
    \textbf{\texttt{[20]}} & \citet{Jingjing}                        & \english\\
    % 2020
    \textbf{\texttt{[21]}} & \citet{liu}                             & \english \\
    % 2021
    \textbf{\texttt{[22]}} & \citet{styleptb}                        & \english \\
    % 2021
    \textbf{\texttt{[23]}} & \citet{xformal}                         &  \portuguese, \french, \italian \\

    \end{tabular}}
    \caption{List of prior works on \fost along with languages (i.e., \texttt{iso} codes) addressed in each of them.}\vspace{-0.5cm}
    \label{tab:status_mapping}
\end{table}
